DMLO: Deep Matching LiDAR Odometry

LiDAR odometry is a fundamental task for various areas such as robotics, autonomous driving. This problem is difficult since it requires the systems to be highly robust running in noisy real-world data. Existing methods are mostly local iterative methods. Feature-based global registration methods are not preferred since extracting accurate matching pairs in the nonuniform and sparse LiDAR data remains challenging. In this paper, we present Deep Matching LiDAR Odometry (DMLO), a novel learning-based framework which makes the feature matching method applicable to LiDAR odometry task. Unlike many recent learning-based methods, DMLO explicitly enforces geometry constraints in the framework. Specifically, DMLO decomposes the 6-DoF pose estimation into two parts, a learning-based matching network which provides accurate correspondences between two scans and rigid transformation estimation with a close-formed solution by Singular Value Decomposition (SVD). Comprehensive experimental results on real-world datasets KITTI and Argoverse demonstrate that our DMLO dramatically outperforms existing learning-based methods and comparable with the state-of-the-art geometry based approaches.

==> src/experiments.tex <==


\begin{table*}[!t]
	\centering
		\caption{Odometry results on KITTI odometry dataset~\cite{geiger2013vision}. Here $t_{rel}$ is translation errors(\%) on all possible subsequences of 100m-800m. $r_{rel}$ is rotational error($^\circ$/100m) on the length of 100m-800m. }
		\label{tab:kitti}
		\scalebox{0.9}{
		\begin{tabular}{l | c c | c c | c c | c c| c c| c c| c c| c c}
		 \toprule
		 & \multicolumn{2}{c|}{ICP-po2po} & \multicolumn{2}{c|}{ICP-po2pl}  & \multicolumn{2}{c|}{GICP~\cite{segal2009generalized}}  & \multicolumn{2}{c|}{CLS~\cite{velas2016collar}} & \multicolumn{2}{c|}{SUMA~\cite{behley2018efficient}}  & \multicolumn{2}{c|}{LOAM~\cite{zhang2014loam}}& \multicolumn{2}{c|}{Ours}  & \multicolumn{2}{c}{Ours+Mapping}  \\
		 Seq & $t_{rel}$ & $r_{rel}$  & $t_{rel}$ & $r_{rel}$ & $t_{rel}$ & $r_{rel}$ & $t_{rel}$ & $r_{rel}$ & $t_{rel}$ & $r_{rel}$ & $t_{rel}$ & $r_{rel}$  & $t_{rel}$ & $r_{rel}$  & $t_{rel}$ & $r_{rel}$\\
		 \midrule
		$00$ & 6.88  & 2.99 & 3.80 &1.73& 1.29  & 0.64 & 2.11 & 0.95 & \textbf{0.68} & \textbf{0.23} & 0.78 & 0.53 & 0.83 & 0.44 & 0.73 &0.44\\
		$01$ & 11.21 & 2.58 & 13.53&2.58& 4.39  & 0.91 & 4.22 & 1.05 & 1.70 & \textbf{0.54} & \textbf{1.43} & 0.55 & 3.14 & 1.15 & 1.91 &\textbf{0.54}\\
		$02$ & 8.21  & 3.39 & 9.00 &2.74& 2.53  & 0.77 & 2.29 & 0.86 & 1.20 & \textbf{0.48} & \textbf{0.92} & 0.55 & 1.08 & 0.53 & 1.01 &0.58\\
		$03$ & 11.07 & 5.05 & 2.72 &1.63& 1.68  & 1.08 & 1.63 & 1.09 & \textbf{0.74} & 0.50 & 0.86 & 0.65 & 0.80 & \textbf{0.49} & 1.06 &0.53\\
		$04$ & 6.64  & 4.02 & 2.96 &2.58& 3.76  & 1.07 & 1.59 & 0.71 & \textbf{0.44} & \textbf{0.27} & 0.71 & 0.50 & 0.71 & 0.53 & 0.61 &0.66\\
		$05$ & 3.97  & 1.93 & 2.29 &1.08& 1.02  & 0.54 & 1.98 & 0.92 & \textbf{0.43} & \textbf{0.20} & 0.57 & 0.38 & 0.90 & 0.46 & 0.65 &0.33\\
		$06$ & 1.95  & 1.59 & 1.77 &1.00& 0.92  & 0.46 & 0.92 & 0.46 & \textbf{0.54} & \textbf{0.30} & 0.65 & 0.39 & 0.91 & 0.46 & 0.65 &0.34\\
		$07$ & 5.17  & 3.35 & 1.55 &1.42& 0.64  & 0.45 & 1.04 & 0.73 & 0.74 & 0.54 & 0.63 & \textbf{0.50} & 0.58 & 0.51 & \textbf{0.53} &0.51\\
		$08$ & 10.04 & 4.93 & 4.42 &2.14& 1.58  & 0.75 & 2.14 & 1.05 & 1.20 & \textbf{0.38} & 1.12 & 0.44 & 1.02 & 0.48 & \textbf{0.93} &0.48\\
		$09$ & 6.93  & 2.89 & 3.95 &1.71& 1.97  & 0.77 & 1.95 & 0.92 & 0.62 & \textbf{0.22} & 0.77 & 0.48 & 1.02 & 0.45 & \textbf{0.58} &0.30\\
		$10$ & 8.91  & 4.74 & 6.13 &2.60& 1.31  & 0.62 & 3.46 & 1.28 & \textbf{0.72} & \textbf{0.32} & 0.79 & 0.57 & 1.08 & 0.59 & 0.75 &0.52\\
		\midrule
		\text{mean} & 7.37  & 3.40 & 4.72 & 1.93 & 1.92 & 0.73 & 2.12 & 0.91 & \textbf{0.83} & \textbf{0.36} & 0.84 & 0.50 & 1.09    & 0.55    & 0.85    &  0.47   \\
		 \bottomrule
		\end{tabular}
		}
		\vspace{-3mm}
\end{table*}

\begin{figure*}[!t]
    \centering
    \begin{tabular}{cc}
		\includegraphics[width=0.45\linewidth]{pics/used/07-1.png} &
		\includegraphics[width=0.45\linewidth]{pics/used/08-1.png} \\
		(a) sequence 07  & (b) sequence 08 \\
		\includegraphics[width=0.45\linewidth]{pics/used/09-1.png} &
		\includegraphics[width=0.45\linewidth]{pics/used/10-1.png} \\
		 (c) sequence 09  & (d) sequence 10 \\
		\end{tabular}
    \caption{Qualitative results on the testing sequences of KITTI odometry dataset~\cite{geiger2013vision}.}
    \label{fig:qualitative}
    \vspace{-5mm}
\end{figure*}

\section{Experiments}\label{sec:exp}
In this section, we report the results of our DMLO method. We will briefly introduce the datasets we use first, then followed by odometry results and registration results under large motion. Finally, we conduct ablation studies to demonstrate the impact of each component in our system.
\subsection{Datasets}
\paragraph{KITTI}
The KITTI odometry benchmark~\cite{geiger2013vision, geiger2012we} provides 4 camera images, Velodyne HDL-64E LiDAR scans,
and 6-DoF ground truth pose from a high accuracy integrated GPS/IMU system. %It contains 21 sequences with 43552 frames, 11 sequences (00-10) associated with ground truth trajectories and 11 sequences (11-21) without ground truth for online evaluation.
The dataset was recorded at 10fps when driving in highways, country roads and urban areas.
It is the most widely used LiDAR odometry benchmark in the literature.

\paragraph{Argoverse}
Argoverse 3D tracking dataset~\cite{Argoverse} is a recently proposed dataset tailored for autonomous driving.
It contains 360-degree images from 7 cameras, forward-facing stereo cameras, 3D point clouds from LiDAR and 6-DoF ego-localization for each timestamp.
The whole dataset consists of 100 sequences varying in length from 15 to 60 seconds collected in two US cities with more moving objects than KITTI.
Different from KITTI, the point cloud is captured with two roof-mounted VLP-32 LiDAR sensors
with an overlapping $40^\circ$ vertical field of view. We use this dataset to demonstrate the robustness of our method to different hardware configurations.%Fig.n shows the difference in cylinder image.

\subsection{Implementation Details}
In KITTI dataset, we use the resolution from Velodyne HDL-64 specs and set $\Delta\phi=0.4^\circ, \Delta\theta=0.2^\circ$ in \equref{eqn:projection}. So that the size of cylinder frames is $H=68, W=1801$ with $26.9^\circ, 360^\circ$ FOV in vertical, horizontal. For network inputs, we crop it to $64\times 1792$ from the center because of the sparsity in the edge. In Argoverse dataset, since the two overlapping VLP-32 LiDAR make the distribution of point cloud denser in middle areas and sparser on both sides, we set a smaller vertical resolution as $\Delta\phi=0.3^\circ$ within $20^\circ$ FOV while keeping the horizontal resolution as $\Delta\theta=0.2^\circ$.

During training, we first sample a set of three successive scans, and for each three scans, we use it to form three training pairs $[S_{t-1}, S_t], [S_t, S_{t+1}]$ and $[S_{t-1}, S_{t+1}]$ as training samples. The reason for forming the last one by skipping one scan is to augment the training with large displacement.  All models are trained using SGD with momentum of 0.9 for 60 epochs. The learning rate is set to $0.0005$ at beginning and multiplied by 0.1 every 20 epochs with $10^{-5}$ weight decay. The batch size is 32 and 8 NVIDIA 1080Ti GPU is used to train the models with synchronized batch normalization (SyncBN)~\cite{zhang2018context}. The whole framework is implemented with the MXNet library~\cite{chen2015mxnet}. For inference, we set $r=1$ in NMS to keep the correspondences spatial uniformly distributed. And the inlier threshold in RANSAC is 0.1m. If the inliners correspondences are less than 10, we will use the result from motion model.

\subsection{Odometry Results}

On KITTI dataset, we compare our methods with two kinds of odometry estimation methods. Geometry-based methods: point-to-point ICP (ICP-po2po), point-to-plane ICP (ICP-po2pl), GICP~\cite{segal2009generalized}, CLS~\cite{velas2016collar} and LOAM~\cite{zhang2014loam}; Learning-based methods: DeepLO~\cite{cho2019deeplo}, LO-Net~\cite{li2019net} and Velas \etal~\cite{velas2018cnn}. All the methods are evaluated by official evaluation metrics. The three learning-based methods have different training/testing split, DeepLO uses 00-08/09-10, Velas uses 00-07/08-10, LO-Net uses 00-06/07-10 as training/testing, respectively. For fair comparison, we follow the setting of LO-Net which requires the least training data.

\tabref{tab:DL-KITTI} shows testing results of all these learning-based networks, ours consistently outperforms the others by a large margin even with less training data. To fairly evaluate the performance of our DMLO in all sequences with other geometric based methods, we train our DMLO in leave-on-out manner. For example, to test sequence 00, we train our network on 01-10. We report both results of our method with and without backend mapping refinement. We compare the results with these methods in \tabref{tab:kitti}. Compared with pure odometry method, our DMLO significantly outperforms the baselines ICP and GICP, while compared with other full SLAM systems, DMLO demonstrates competitive or better results. \emph{Note that this is the first feature-based global method could compete with LOAM.} A qualitative results has been visualized in \figref{fig:qualitative}.


\begin{table}[!t]
	\centering
		\caption{Comparison of learning-based methods in KITTI~\cite{geiger2013vision}. We only show the results in testing split.}
		\label{tab:DL-KITTI}
		\scalebox{0.85}{
		\begin{tabular}{l | c c | c c| c c| c c}
		 \toprule
		 & \multicolumn{2}{c|}{~\cite{velas2018cnn}} & \multicolumn{2}{c|}{DeepLO\cite{cho2019deeplo}}  & \multicolumn{2}{c}{LO-Net~\cite{li2019net}} & \multicolumn{2}{c}{Ours}\\
		 Seq. & $t_{rel}$ & $r_{rel}$ & $t_{rel}$ & $r_{rel}$  & $t_{rel}$ & $r_{rel}$& $t_{rel}$ & $r_{rel}$\\
		 \midrule
		07 & -    & - & - & - & 1.70 & 0.89 & \textbf{0.73} & \textbf{0.48} \\
		08 & 2.89 & - & - & - & 2.12 & 0.77 & \textbf{1.08} & \textbf{0.42}\\
		09 & 4.94 & - & 13.35 & 4.45 & 1.37 & 0.58 & \textbf{1.10} & \textbf{0.61}\\
		10 & 3.27 & - & 5.83 & 3.53 & 1.75 & 0.79 & \textbf{1.12} & \textbf{0.64}\\
		
		 \bottomrule
		\end{tabular}
		}
		\vspace{-3mm}
	\end{table}


% As LO-Net setting, we split sequence 00-06/07-10 for training/testing and evaluate all methods using official evaluation metrics. \tabref{tab:kitti} shows the results on KITTI, where our network achieves the state-of-the-art performance in learning-based methods. And our full method is comparable to LOAM and LO-Net+Mapping.

On the Argoverse dataset, we only compare with ICP-po2po, GICP and NDT, because LOAM is infeasible to apply on two VLP-32 LiDAR.
We evaluate the performance of all the methods on the official training/testing split. Since most sequences in Argoverse are shorter than 200 frames, the metrics from KITTI are not suitable. As ~\cite{sturm2012benchmark} suggests, we use Absolute Trajectory Error(ATE) and Relative Pose Error(RPE) to evaluate the accuracy.
%The RPE measures the local accuracy of the trajectory by comparing relative pose differences between estimated and ground truth. And ATE evaluates the global consistency in an odometry system by computing the absolute distance in every timestamp.
\tabref{tab:argo} shows that our proposed method outperforms the others remarkably both in terms of ATE and RPE.

\begin{table}[!t]
	\centering
		\caption{Odometry experiments on Argoverse dataset~\cite{Argoverse}. Our DMLO outperforms other methods even in different hardware(two VLP-32 LiDAR).}
		\label{tab:argo}
		\scalebox{1.0}{
		\begin{tabular}{l | c c | c c}
		 \toprule
		 & \multicolumn{2}{c|}{RPE} & \multicolumn{2}{c}{ATE} \\
		 Methods & Mean & Max & Mean & Max \\
		 \midrule
		ICP-Po2Po & 0.12 & 0.35 & 10.22 & 27.59 \\
		G-ICP & 0.05 & 0.21 & 3.74 & 15.94 \\
		NDT-P2D & 0.11  & 0.37 & 4.33 & 17.03 \\
		\midrule
		 Ours  & \textbf{0.01}  & \textbf{0.10} & \textbf{0.57} & \textbf{1.91} \\
		 \bottomrule
		\end{tabular}
		}
		\vspace{-3mm}
\end{table}

\begin{table}[!htb]
	\centering
		\caption{Registration experiments in KITTI~\cite{geiger2013vision}.}
		\label{tab:registration}
		\scalebox{0.9}{
		\begin{tabular}{l | c c | c c}
		 \toprule
		 & \multicolumn{2}{c|}{Angular Error($^\circ$)} & \multicolumn{2}{c}{Translation Error(m)} \\
		Methods  & Mean & Max & Mean & Max \\
		 \midrule
		ICP-Po2Po & 0.139 & 1.176 & 0.089 & 2.017 \\
		ICP-Po2Pl & 0.084 & 1.693 & 0.065 & 2.050 \\
		G-ICP & 0.067 & 0.375 & 0.065 & 2.045 \\
		AA-ICP & 0.145 & 1.406 & 0.088 & 2.020 \\
		NDT-P2D & 0.101  & 4.369 & 0.071 & 2.000 \\
		CPD & 0.461  & 5.076 & 0.804 & 7.301 \\
		\midrule
		3DFeat-Net & 0.199  & 2.428 & 0.116 & 4.972 \\
		DeepVCP & 0.164  & 1.212 & 0.071 & \textbf{0.482} \\
		 \midrule
		 Ours  & \textbf{0.021}  & \textbf{0.070} & \textbf{0.060} & 0.830 \\
		 \bottomrule
		\end{tabular}
		}
		\vspace{-3mm}
	\end{table}

% To be refine
\begin{table}[]
	\centering
	\setlength{\tabcolsep}{6pt}
	\vspace{2mm}
	\caption{End Point Error(EPE) and percentage of outliers averaged over all ground truth pixels(Fl-all) in KITTI 07-10 sequences. The table shows the different results of Feature Normalized(FN), Subpixel(S) loss and Deformable(D) conv.}\label{tab:ablation1}
	\begin{tabular}{l|c|c|c}
		\toprule
		Methods    & Model     & EPE(pixel) & Fl-all(\%) \\ \midrule
		Basic & 5conv & 0.57 & 6.7 \\
		Basic+FN & 5conv & 0.55 &  6.1 \\
		Basic+FN+S & 5conv &  0.52 & 5.6  \\
		\midrule
		Basic+FN+S & 8conv & 0.49 & 5.2 \\
		Basic+FN+S & 2conv+3D & \textbf{0.45} & \textbf{4.2} \\
		\bottomrule
	\end{tabular}
	
	\vspace{-3mm}
\end{table}

\begin{table}[!t]
	\centering
		\caption{The effect of Motion Model (MM) and Moving Objects Removal (OR) on KITTI. The mean of translation and rotation error are computed as \tabref{tab:kitti}. $\text{mean}^\dagger$ is mean of the results in the training set and $\text{mean}^*$ is that in testing set.}
		\label{tab:ablation2}
		\scalebox{1.0}{
		\begin{tabular}{l | c c | c c| c c}
		 \toprule
		 & \multicolumn{2}{c|}{Basic} & \multicolumn{2}{c|}{Basic+MM}  & \multicolumn{2}{c}{Basic+MM+OR}\\
		 Seq. & $t_{rel}$ & $r_{rel}$ & $t_{rel}$ & $r_{rel}$  & $t_{rel}$ & $r_{rel}$\\
		 \midrule
		$\text{mean}^\dagger$ & 1.66 & 0.59 & 1.24 & 0.58  & \textbf{1.16} & \textbf{0.57}\\
        $\text{mean}^*$ & 0.97 & 0.54 & \textbf{0.96} & 0.57 & 1.00 & \textbf{0.53} \\
		 \bottomrule
		\end{tabular}
		}
		\vspace{-3mm}
\end{table}
\subsection{Registration under Large Motion}
Although our network is not designed to large scale registration, we also report the results comparing with recent proposed learning-based methods such 3DFeat-Net~\cite{yew20183dfeat} and DeepVCP~\cite{Lu_2019_ICCV}. For registration, we simply change the max-displacement $D$ in coarse level from $10 \times 10$ to $40\times 40$ in inference time without fine-tuning. Following DeepVCP, we sample the scans at 30 frame intervals and use all frames within 5m distance to it as registration target. The angular error and translation error is used to compare the performance of all methods. Given ground-truth transformation $(\overline{\bf{R}}, \overline{\bf{t}})$ and prediction $(\bf{R}, \bf{t})$, the translation error is defined as $\left \|\bf{t}-\overline{\bf{t}}\right \|_2$ and angular error as $\theta=2\arcsin(\frac{\left\|\bf{R}-\overline{\bf{R}}\right\|_F}{2\sqrt{2}})$. The results in \tabref{tab:registration} indicate that, though we only use neighbor frames for training, our network can still generalize to distant registration task without any further tuning.


\subsection{Ablation Study} \label{sec:ablation}
In this section, we conduct a set of ablation studies to understand how each component affects our performance. We first validate the efficacy of different network modules in the refinement network  described in \secref{subsec:architectures}. Then we experiment with and without motion model and moving objects removal. We utilize KITTI dataset in this section.

 \tabref{tab:ablation1} shows that the Feature Normalized(FN), Subpixel(S) loss and Deformable(D) convolution significantly improve the accuracy of network. Specifically, the experiments between deeper network and deformable convolution clearly show that adaptive receptive field is essential for matching. Adopting deformable convolution is more economical than simply adding more plain convolution layers.

 \tabref{tab:ablation2} describes how the Motion Model(MM) and Moving Objects Removal(OR) affect our methods. As we can see, the influence of MM and OR on training set is greater than that on testing set. It is because sequence 01 in training set is recorded in highway with continuous featureless area and high speed. \tabref{tab:kitti} also verifies that 01 is the most challenging sequence in all 11 sequences.




